Hierarchical Imitation Learning of Team Behavior from Heterogeneous Demonstrations

Successful collaboration requires team members to stay aligned, especially in complex sequential tasks. Team members must dynamically coordinate which subtasks to perform and in what order. However, real-world constraints like partial observability and limited communication bandwidth often lead to suboptimal collaboration. Even among expert teams, the same task can be executed in multiple ways. To develop multi-agent systems and human-AI teams for such tasks, we are interested in data-driven learning of multimodal team behaviors. Multi-Agent Imitation Learning (MAIL) provides a promising framework for data-driven learning of team behavior from demonstrations, but existing methods struggle with heterogeneous demonstrations, as they assume that all demonstrations originate from a single team policy. Hence, in this work, we introduce DTIL: a hierarchical MAIL algorithm designed to learn multimodal team behaviors in complex sequential tasks. DTIL represents each team member with a hierarchical policy and learns these policies from heterogeneous team demonstrations in a factored manner. By employing a distribution-matching approach, DTIL mitigates compounding errors and scales effectively to long horizons and continuous state representations. Experimental results show that DTIL outperforms MAIL baselines and accurately models team behavior across a variety of collaborative scenarios.

==> math_symbols.tex <==
\usepackage{bbm}

\newcommand\myeq{\mkern1.5mu{=}\mkern1.5mu} 
\newcommand\mycol{\mkern1.5mu{:}\mkern1.5mu} 
\newcommand\mysum{\mkern1.5mu{+}\mkern1.5mu}
\newcommand\mypm{\mkern1.5mu{\pm}\mkern1.5mu} 
\newcommand{\xhat}{\hat{x}} 

\newcommand{\MS}[2]{\begin{tabular}{l}#1$\mypm$#2\end{tabular}}


% fields
\newcommand{\field}[1]{\mathbb{#1}}
\newcommand{\N}{\field{N}} 
\newcommand{\R}{\field{R}} 
\newcommand{\C}{\field{C}} 
\newcommand{\F}{\field{F}} 

% special operators
\DeclareMathOperator{\EX}{\ensuremath{\mathbb{E}}}  % expected value
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

% function symbols
\newcommand{\Ind}{\mathbbm{1}}  % indicator function

% braces
\newcommand{\Set}[3]{\{#1\}_{#2}^{#3}} 

% caligraphic
\newcommand{\calM}{\mathcal{M}}
\newcommand{\calN}{{\mathcal{N}}}
\newcommand{\calD}{\mathcal{D}}
\newcommand{\calC}{\mathcal{C}}

% bar
\newcommand{\barA}{\bar{A}}

% tilde
\newcommand{\tilpi}{{\tilde{\pi}}}
\newcommand{\tilcalD}{{\tilde{\calD}}}
\newcommand{\tilD}{{\tilde{D}}}

% hat
\newcommand{\hatChi}{{\hat{\chi}}}
\newcommand{\hatX}{{\hat{x}}}

% check
\newcommand{\chkRho}{{\check{\rho}}}

% grave
\newcommand{\grvRho}{{\grave{\rho}}}

% for concatenating two subscripts
\newcommand{\concat}[2]{
\expandafter\ifx\expandafter\relax\detokenize{#1}\relax   % first is empty
    \expandafter\ifx\expandafter\relax\detokenize{#2}\relax  % second is empty
        {}
    \else  % second not empty
        {#2}
    \fi
\else  % first not empty
    \expandafter\ifx\expandafter\relax\detokenize{#2}\relax  % second is empty
        {#1}
    \else
        {#1, #2}
    \fi
\fi
}

% model symbols 
\newcommand{\Prev}[1]{{#1}^{-}}  % previous [action, intent, ...]
\newcommand{\Next}[1]{{#1}'}  % next [state, intent ...]
\newcommand{\Joint}[1]{#1}  % joint [action, obs, intent, ...]
\newcommand{\Others}[2]{{#1}_{-#2}}  % others' [action, intent, ...]
\newcommand{\AtTime}[2]{{#1}^{#2}}  % at time t

\newcommand{\obs}{o}
\newcommand{\Tx}{\zeta}  % intent transition

\newcommand{\ExtA}{A^{+}}  % extended action set
\newcommand{\ExtX}{X^{+}}  % extended intent set

\newcommand{\PrA}[1]{\Prev{a}_{#1}}  % previous action
\newcommand{\PrX}[1]{\Prev{x}_{#1}}  % previous intent

\newcommand{\NxA}[1]{\Next{a}_{#1}}  % next action
\newcommand{\NxS}{\Next{s}}  % next state

\newcommand{\JoA}{\Joint{a}}  % joint action
\newcommand{\JoX}{\Joint{x}}  % joint intent
\newcommand{\JoO}{\Joint{\obs}}  % joint observation

\newcommand{\PrJoA}{\Prev{\Joint{a}}}  % previous joint action
\newcommand{\PrJoX}{\Prev{\Joint{x}}}  % previous joint intent

\newcommand{\OtA}[1]{\Others{a}{#1}}  % others' action
\newcommand{\OtX}[1]{\Others{x}{#1}}  % others' intent

\newcommand{\PrOtA}[1]{\Prev{\OtA{#1}}}  % others' previous actions

\newcommand{\TmOtA}[2]{\AtTime{\OtA{#1}}{#2}}  % others' action at time t
\newcommand{\TmA}[2]{\AtTime{a_{#1}}{#2}}  % action at time t
\newcommand{\TmX}[2]{\AtTime{x_{#1}}{#2}}  % intent at time t
\newcommand{\TmO}[2]{\AtTime{\obs_{#1}}{#2}}  % observation at time t
\newcommand{\TmS}[1]{\AtTime{s}{#1}}  % state at time t
\newcommand{\TmJoO}[1]{\AtTime{\JoO}{#1}}  % joint observation at time t
\newcommand{\TmJoA}[1]{\AtTime{\JoA}{#1}}  % joint observation at time t
\newcommand{\TmOA}[2]{\TmO{#1}{#2}, \TmA{#1}{#2}}
\newcommand{\TmJoOA}[1]{\TmOA{}{#1}}
\newcommand{\TmXEst}[2]{\AtTime{\hatX_{#1}}{#2}}  % intent at time t
\newcommand{\TmOATrj}[2]{(\TmO{#1}{}, \TmA{#1}{})^{#2}}

\newcommand{\piE}{\pi_{E}}
\newcommand{\OtPi}[1]{\Others{\pi}{#1}}
\newcommand{\OtTx}[1]{\Others{\Tx}{#1}}
\newcommand{\OtAM}[1]{\Others{\calN}{#1}}

\newcommand{\JoAM}{\calN_{1:n}}  % we use different representation for this.

% neuralnet
\newcommand{\PiParam}{\theta}  %  pi parameter
\newcommand{\TxParam}{\phi}  % Tx parameter
\newcommand{\PaPi}[2]{{\pi_{\PiParam_{#1}}^{#2}}}  % parameterized pi
\newcommand{\PaTx}[2]{{\Tx_{\TxParam_{#1}}^{#2}}}  % parameterized Tx
\newcommand{\PaAM}[2]{{\calN_{\PiParam_{#1}, \TxParam_{#1}}^{#2}}}  % parameterized agent model
\newcommand{\JoPaAM}[1]{{\calN_{1:n, \PiParam, \TxParam}^{#1}}}  % parameterized agent model
\newcommand{\PaPiTx}[3]{\PaPi{#1}{#2}, \PaTx{#1}{#3}}  % parameterized 

% data symbols
\newcommand{\Traj}[1]{{\tau_{#1}}} 
\newcommand{\TrajTeam}{\Traj{}}
\newcommand{\Demo}[1]{{D_{#1}}}
\newcommand{\DemoTeam}{\Demo{}}
\newcommand{\DemoX}[1]{\tilD_{#1}}
\newcommand{\DemoTeamX}{\DemoX{}}
\newcommand{\Rollout}[1]{{{R}_{#1}}}  % collection of rollouts
\newcommand{\RolloutTeam}{{\Rollout{}}}

\newcommand{\XSeq}[1]{\chi_{#1}}
\newcommand{\XEstSeq}[1]{\hatChi_{#1}}
% \newcommand{\XLabel}[1]{\{x_{#1}^{i_1}, \cdots, x_{#1}^{i_k}\}}
\newcommand{\XLabel}[3]{\{\XSeq{#1}\}_{#2}^{#3}}
\newcommand{\XEst}[3]{\{\XEstSeq{#1}\}_{#2}^{#3}}

\newcommand{\TrajX}[1]{{\bar{\tau}_{#1}}} 

% loss
\newcommand{\Lam}{L_{oaxx}}  % loss for agent model
\newcommand{\Lpi}[2]{{L_{oax, #1}}^{#2}}  % loss for policy
\newcommand{\Ltx}[2]{{L_{oxx, #1}}^{#2}}  % loss for intent transition
\newcommand{\Loss}[1]{L^{#1}}  % loss 

% input signature
\newcommand{\oaxx}[1]{\obs_{#1}, a_{#1}, x_{#1}, \PrX{#1}}
\newcommand{\oax}[1]{\obs_{#1}, a_{#1}, x_{#1}}
\newcommand{\oxx}[1]{\obs_{#1}, x_{#1}, \PrX{#1}}

\newcommand{\OMamEst}[3]{\rho_{#1}^{#3}(\oaxx{#2})}
\newcommand{\OMpiEst}[3]{\rho_{#1}^{#3}(\oax{#2})}
\newcommand{\OMtxEst}[3]{\rho_{#1}^{#3}(\oxx{#2})}

% occupancy measure
\newcommand{\OMam}[2]{\OMamEst{#1}{#2}{}}
\newcommand{\OMamCon}[3]{\rho_{#1}(\oaxx{#2}|#3)}
\newcommand{\OMpi}[2]{\OMpiEst{#1}{#2}{}}  % occupancy measure with oax input
\newcommand{\OMtx}[2]{\OMtxEst{#1}{#2}{}}
\newcommand{\OMdot}[1]{\rho_{#1}(\cdot)}

\newcommand{\OMtwoEst}[6]{\rho_{#3}^{#6}({#1}_{#4}, {#2}_{#5})}
\newcommand{\OMtwo}[5]{\OMtwoEst{#1}{#2}{#3}{#4}{#5}{}}

\newcommand{\OMsa}[2]{\OMtwo{s}{a}{#1}{}{#2}}
% \newcommand{\OMsa}[2]{\rho_{#1}(s, a_{#2})}
\newcommand{\OMsaxx}[1]{\rho_{#1}(s, a, x, \PrX{})}

\newcommand{\sumUnP}[1]{\sum_{t=0}^\infty \gamma^t p(#1)}
\newcommand{\sumP}[1]{(1-\gamma)\sumUnP{#1}}

% divergence
\newcommand{\Dfam}[4]{D_f\left(\OMam{#1}{#3} \middle|\middle| \OMamEst{#2}{#3}{#4}\right)}
\newcommand{\Dfamchk}[4]{D_f\left(\OMam{#1}{#3} \middle|\middle| \chkRho_{#2}^{#4}(\oaxx{#3})\right)}
\newcommand{\Dfamgrv}[4]{D_f\left(\OMam{#1}{#3} \middle|\middle| \grvRho_{#2}^{#4}(\oaxx{#3})\right)}
\newcommand{\Dfpi}[4]{D_f\left(\OMpi{#1}{#3} \middle|\middle| \OMpiEst{#2}{#3}{#4}\right)}
\newcommand{\Dftx}[4]{D_f\left(\OMtx{#1}{#3} \middle|\middle| \OMtxEst{#2}{#3}{#4}\right)}
\newcommand{\Dfdot}[2]{D_f\left(\OMdot{#1} \middle|\middle| \OMdot{#2}\right)}
\newcommand{\Dfsa}[3]{D_f\left(\OMsa{#1}{#3} \middle|\middle| \OMsa{#2}{#3}\right)}
\newcommand{\Dfsaxx}[2]{D_f\left(\OMsaxx{#1} \middle|\middle| \OMsaxx{#2}\right)}

\newcommand{\Df}[3]{D_f\left({#1}(#3) \middle|\middle| {#2}(#3)\right)}

\newcommand{\Dftwo}[6]{D_f\left(\OMtwo{#1}{#2}{#3}{#5}{#5} \middle|\middle| \OMtwoEst{#1}{#2}{#4}{#5}{#5}{#6}\right)}

% rho 
\newcommand{\rhoE}{\rho_{E}}
\newcommand{\rhopi}{\rho_{\pi}}
\newcommand{\rhotx}{\rho_{\Tx}}
\newcommand{\rhoam}{\rho_{\calN}}


% new states & action
\newcommand{\Spi}{u}
\newcommand{\Stx}{v}
\newcommand{\Sam}{\Stx}
\newcommand{\Aam}{w}


